Shapeception: Unravelling Brain Activity during Animated Shape Perception and Mentalization

In this paper, we investigate the brain activity elicited during perception of animated shapes as stimuli, which have been found to evoke mental state attributions. Contrary to a previous study, we incorporated the participants' responses in the analysis, and observed robust activations in mPFC, which has been found to play an important role in understanding other's and one's own nature. From our analyses, TPOj was observed showing robust activation during the task as well as functionally connected to AA and LTC, which lead to speculation that empathy might co-occur with mentalizing in the task and that humans might be able to empathize with these interacting shapes, in spite of lacking human features. Along with this, in one of our analyses, we were able to localize a region close to the pSTS, where the activation depicted the participants' 'ability to mentalize'. Based on our observations, we modelled the prediction of mentalization and propose our model as an approach towards developing a brain-activity based model to detect ToM (Theory of Mind) difficulties, which could be useful in research about disorders like Autism Spectrum Disorder (ASD) as well as assessment of mentalization-based treatments. Additionally, we use our findings to reiterate how the Resting State might not always act as a good control condition and that control conditions should be task-specific.

==> ToDo.tex <==
Case lines improve
Explain figures
% Experiment design diagram














Minaxi
1. We can also report descriptive stats- from 339, how many were able to correctly classify - or mentalize and then from these what was the proportion of whom were able to empathize.

% 2. We can add Conclusion (or Summary) and a Limitations & discussions section. 

% 3. Add labels to brain plots.

% 4. Discuss on difference between the three - M, E, ToM

% 5. See intersection and divergence paper - for linking.

% 6. Highlight the novel findings and bring story accordingly
%     % - Main paper - considering responses - as a control
%     - The third region
%     - We can write our whole story in terms of our novel findings, as in what we have found in literature and what we have improved on
% 7. citations as remaining places
% 8. TPO -> TPj everywhere and make short forms
9. Check in correlation later
title
% abstract
% discussion
% remove from analysis

% captions in figures
% ROI
% Case ABC

Varad
1. Check if the figshare citation is correct
2. labelling parts 

-------------------------------

% Keyowrds: Machine Learning; empathy, mentalising, moving shapes

% - Does mentalising even mean empathising?
% - Mentalising leads to empathising
% - Modelling fMRI activity to predict mentalising
% - Do we have specific regions for empathy?
% - Can empathy be learned?
% - Can moving shapes help learn empathy?
% - Interpreting the moving shapes
% - Judging shape interaction

------------------------------------------

-> for 7 pages
Add analyses description
add mirroring in discussion
Change caption fif 3 -> activations in network activations

